climber++: Pivot-Based Approximate Similarity Search over Big Data Series

The generation and collection of big data series are becoming an integral part of many emerging applications in sciences, IoT, finance, and web applications among several others. The terabyte-scale of data series has motivated recent efforts to design fully distributed techniques for supporting operations such as approximate kNN similarity search, which is a building block operation in most analytics services on data series. Unfortunately, these techniques are heavily geared towards achieving scalability at the cost of sacrificing the results' accuracy. State-of-the-art systems report accuracy below 10% and 40%, respectively, which is not practical for many real-world applications. In this paper, we investigate the root problems in these existing techniques that limit their ability to achieve better a trade-off between scalability and accuracy. Then, we propose a framework, called CLIMBER, that encompasses a novel feature extraction mechanism, indexing scheme, and query processing algorithms for supporting approximate similarity search in big data series. For CLIMBER, we propose a new loss-resistant dual representation composed of rank-sensitive and ranking-insensitive signatures capturing data series objects. Based on this representation, we devise a distributed two-level index structure supported by an efficient data partitioning scheme. Our similarity metrics tailored for this dual representation enables meaningful comparison and distance evaluation between the rank-sensitive and ranking-insensitive signatures. Finally, we propose two efficient query processing algorithms, CLIMBER-kNN and CLIMBER-kNN-Adaptive, for answering approximate kNN similarity queries. Our experimental study on real-world and benchmark datasets demonstrates that CLIMBER, unlike existing techniques, features results' accuracy above 80% while retaining the desired scalability to terabytes of data.

==> misc <==
% \begin{figure}[t]
%   \centering
%   \begin{subfigure}[t]{0.49\columnwidth}
%       \centering
%       \includegraphics[width=1.0\textwidth]{fig/4ps_index.pdf}
%       \caption{4Ps-index}
%       \label{fig:4ps-index}
%   \end{subfigure}%
%   ~
%   \begin{subfigure}[t]{0.49\columnwidth}
%       \centering
%       \includegraphics[width=1.0\textwidth]{fig/group-structure.pdf}
%       \caption{Group Structure}
%       \Description{10}
%       \label{fig:group-structure}
%   \end{subfigure}%
%   \vspace{-2mm}
%   \caption{4Ps Index Structure}
%   \label{fig:index}
%   \vspace{-4mm}
% \end{figure}



% \begin{definition}
%   \textit{\textbf{[Storage Partition]} Given a data series group $G$,  A data series partition $T_t = \langle X_{1}, X_{2}, \cdots, X_{n'} \rangle$ is a subset of $G$. It is the . The partition id $t$ can be mapped to the storage location.}
% \end{definition}

A data series partition $T_m = \lbrace m, \langle (k_1,X_1),$ $\cdots \rangle \rbrace$ is comprised of a metadata value ``m'' and a collection of elements in the form of $(k_i, X_i)$, where $k_i$ is a unique key for its data series object $X_i$.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.75\columnwidth]{fig/group-dist.pdf}
  \caption{Group Distribution Example, $m=3$}
  \Description{1}
  \label{fig:group-dist}
\end{figure}


At the best of our knowledge

Indeed,  the  most  commonly  used  permutation  dis-tance: Spearman’s rho, is a monotonic transformation (squar-ing) of the Euclidean distance. 



First, with the advanced data collection and man-agement technologies, nowadays there are a large num-ber of applications with data sets about gigabytes,terabytes or even petabytes. Such massive data setsnecessarily reside on disks or tapes, making even afew accesses of the base data sets comparably slow.In many cases, precision to ‘‘last decimal’’ is not re-quired for a query answer. Quick approximation withsome error guarantee (e.g., the resident population inAustralia 21,126,700 +∕200) is adequate to provideinsights about the data.Second, decision support system (DSS) and datamining are popular approaches to analyzing large data-bases for decision making. The main characteristic ofthe DSS is that aggregation queries (e.g., count, sum,avg, etc.) are executed on large portion of the data-bases, which can be very expensive and resource inten-sive even for a single analysis query. Due to theexploratory nature of decision making, iterative pro-cess involves multiple query attempts. Approximateanswers with fast response time gives users the abilityto focus on their explorations and quickly identifytruly interesting data. It provides a great scalability ofthe decision support applications.Third, approximate query processing is also used toprovide query preview. In most cases, users are onlyinterested in a subset of the entire database. Given atrial query, query preview provides an overview aboutthe data distribution. The users can preview the num-ber of hits and refine the queries accordingly. Thisprevents users from fruitless queries such as zero-hitsor mega-hits


 This work was supported by the [...] Research Fund of [...] (Number [...]). Additional funding was provided by [...] and [...]. We also thank [...] for contributing [...].

